Siegel Zeros and Sarnak's Conjecture

Assuming the existence of Siegel zeros, we prove that there exists an increasing sequence of positive integers for which Chowla's Conjecture on $k$-point correlations of the Liouville function holds. This extends work of Germ\'an and K\'atai, where they studied the case $k=2$ under identical hypotheses. An immediate corollary, which follows from a well-known argument due to Sarnak, is that Sarnak's Conjecture on M\"obius disjointness holds. More precisely, assuming the existence of Siegel zeros, there exists a subsequence of the natural numbers for which the Liouville function is asymptotically orthogonal to any sequence of topological entropy zero.

==> garbage.tex <==

Let $\lambda$ denote the Liouville function; that is, the completely multiplicative function defined by $\lambda(p):=-1$ for all primes $p$. The Prime Number Theorem (PNT) is equivalent to the fact that $\lambda$ exhibits some cancellation in its partial sums; more precisely,
\begin{align*}
    \sum_{n\leq x} \lambda(n)=o(x),
\end{align*}
as $x\tends \infty$. A famous conjecture due to Chowla \cite{ChowlaConj} states that a similar estimate holds for \textit{multiple correlations} of $\lambda$:

More precisely, assuming the existence of an infinite sequence of Dirichlet characters whose corresponding $L$-functions have exceptional zeros, we obtain upper bounds on the partial sums
    \[
    \sum_{n\leq x}\lambda(n+h_1)\cdots \lambda(n+h_k),
    \]
    for distinct, non-negative integers $h_1,\dots,h_k$, along a subsequence. 
    
    
    \subsection{Controlling the level of distribution}

As mentioned above, the level of distribution is a measure of how well we can control the distribution of $\mathcal{A}$ among the progressions $0\Mod{d}$, for $d|\mathcal{P}.$ In general, one wishes to take $D$ (or, rather, $u$) as large as possible. To simplify matters in our problem, we can do some preliminary sieving, which will allow us to take $D\approx r^{A_x}$, for some $A_x$ going to infinity slowly enough w.r.t. both $x$ and $\eta$:

Using Lemma \ref{Pre-Sieve}, we can restrict ourselves to integers whose $r$-smooth part is $\leq r^{A_x}$, for some $A_x$ to be chosen later. Moreover, this will allow us to take the level of distribution to be $D=r^{A_x}$, so that $u=A_x$ and our goal is to take $A_x$ as large as possible.

\begin{rem}
Strictly speaking, one considers Lemma \ref{FLST} only in the case where $\nu(p)<p$. In our case, it is possible that $\nu(p)=p$, but notice that this does not pose a problem and that the FLST still holds; namely, if $\nu(p)=p$, this essentially means that we are removing all residue classes modulo $p$, so that nothing remains in the set $\mathcal{A}$. In fact, when $\nu(p)=p$, all $s$ are such that $(qa_i^*)s\equiv -(b_i^*+na_i^*)\Mod{p}$, for at least one $i$, so that there is no $m$ such that $\left(\prod_{i=0}^k(b_i^*+na_i^*+mqa_i^*),\prod_{p\leq r}p\right)=1$. 
\end{rem}

What's important to note here is that even if $\nu(p)=p$, this does not stop us from applying Lemma \ref{FLST}: in the case where $\nu(p)=p$, there is no $m$ for which $\left(\prod_{i=0}^k(b_i^*+na_i^*+mqa_i^*),\prod_{p\leq r}p\right) = 1$ (which follows from the fact that $\nu(p)$ counts the number of congruences classes we are removing from the arithmetic progressions modulo $d$ and if we remove all of them, there is nothing left!).

For our purposes, we need slightly more general results, which can be found in \cite{Schmidt}. But, before we can state this more general result, we need to define the notion of \textit{absolute irreducibility}:

\begin{defn}
Given a polynomial $f(x)\in\F_q[x]$, the curve $y^d=f(x)$ is \textbf{absolutely irreducible} iff $y^d=f(x)$ is irreducible over $\F_q$ and over every algebraic extension of $\F_q$.
\end{defn}

\begin{rem}
This definition is typically made to ensure that the curve $y^d=f(x)$ has the "correct" number of $\F_q$-points; see \cite[Theorem 2A]{Schmidt}.
\end{rem}

In principle, the above definition may not be easy to work with, but there are simpler, equivalent statements that one can use; namely,

\begin{lem}[Alternative Definition for Absolutely Irreducible]
\label{AbsIrr}
Suppose the polynomial $y^d=f(x)$ has coefficients in a field $k$. Then the following conditions are equivalent:
\begin{enumerate}
    \item $y^d=f(x)$ is absolutely irreducible;
    \item $y^d=cf(x)$ is absolutely irreducible for every $c\in k,c\neq 0$;
    \item If $f(x)=a(x-x_1)^{d_1}\cdots(x-x_s)^{d_s}$ is the factorization of $f$ in $\overline{k}$ with $x_i\neq x_j$ for $i\neq j$, then $(d,d_1,\dots,d_s)=1$.
\end{enumerate}
\end{lem}
\begin{proof}
See \cite[Lemma 2C]{Schmidt}.
\end{proof}

We can now state the necessary character sum that will be needed for our purposes:


\begin{lem}[Weil Bound]
\label{CharacterSum}
Suppose $\chi$ is a non-principal multiplicative character modulo $q$, of exponent $d|q-1$, with $q$ a prime power. Suppose further that $f(x)\in\F_q[x]$ has degree $m$ and that $y^d=f(x)$ is absolutely irreducible, with $q>100dm^2$. Then,
\[
\sum_{n\Mod{q}}\chi(f(n))\leq 5md^{3/2}q^{1/2},
\]
where the sum runs over a complete residue class modulo $q$.
\end{lem}
\begin{proof}
See \cite[Theorem 2B]{Schmidt}.
\end{proof}

For the main term, we use the fact that the polynomial $P(x):=(b_0^*+a_0^*x)(b_1^*+a_1^*x)\cdots(b_k^*+a_k^*x)$ is absolutely irreducible over $\F_p[x]$ for all $p>k+1$; this follows from Lemma \ref{AbsIrr}, together with the fact $P(x)$ factors into distinct, irreducible factors over $\overline{\F}_p[x]$ iff $a_i^*b_j*\neq a_j^*b_i^*$ in $\overline{\F}_p$ iff $a_ib_i^*\neq a_jb_j^*$ iff $p\nmid (h_i-h_j)$, which follows from the fact that the $a_i$'s are pairwise relatively prime on the primes $p>k+1$. ACTUALLY, NEED TO CONSIDER TWO DIFFERENT CASES: ONE WHERE THE AIS ARE NOT DIVISIBLE BY P AND WHERE EXACTLY ONE AI IS DIVISIBLE BY P.

\begin{rem}
Strictly speaking, Sarnak's conjecture is typically stated for the M{\"o}bius function, but one can move freely between the two, with little to no effort.
\end{rem}

; to see this, note that the $f_\epsilon(n)$'s are already "$\epsilon$-separated" so that at most $\exp(o_{m\rightarrow\infty;\epsilon,f}(m))$ balls are needed to cover these $m$-tuples. So, l



First, let's view the set of $n\in[1,x]$ as a probability space with the uniform probability measure. Then, we're interested in 
\[
\frac{1}{x}\sum_{n\leq x}\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)
=:
\E\left[\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right].
\]

In order to evaluate the above, we first start by considering 
\begin{align*}
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right).
\end{align*}
From Chebyshev's Inequality, this is bounded above by
\[
\frac{1}{(\epsilon m)^{k}}\E\left[\left|\sum_{i=1}^mc_i\lambda(n+i)\right|^{k}\right],
\]
for any $k$ even, which we are free to choose. Then, by expanding this $k$-th power and using the triangle inequality, we have that
\[
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    \leq
    \frac{1}{(\epsilon m)^{k}}\sum_{1\leq i_1,i_2,\dots,i_k\leq m}\E\left[\left|\lambda(n+i_1)\lambda(n+i_2)\cdots\lambda(n+i_k)\right|\right],
\]
which follows by the fact that $|c_i|\leq 1$ for all $i$.

By Chowla's Conjecture, this is $\ll_{\epsilon,m,k}(x)$, unless none of the indices $i_1,\dots,i_k$ is repeated an odd number of times; it remains to count the number of $k$-tuples $(1_i,\dots,i_k)$ for which the indices $i_j$ each have even multiplicity.

Read the indices from left to right and label $i_j$ as "fresh" if $i_j$ is not equal to any of the indices $i_1,\dots,i_{j-1}$ and label $i_j$ as a "repeat" if otherwise. Given $i_1,\dots,i_{j-1}$, there are at most $m$ choices for $i_j$ if $i_j$ is to be fresh and at most $k$ choices if $i_j$ is a repeat. Furthermore, given $i_1,\dots,i_k$, at most $k/2$ indices are fresh (this is because the multiplicity of each $i_j$ must be even, so that fresh indices actually come with a pair further down the line). 

Let $N$ denote the number of fresh indices, so that $k-N$ is the number of repeats. Then, there are $2^km^Nk^{k-N}$ possible $k$-tuples with the desired properties and this is $\leq 2^km^{k/2}k^{k/2}$ as $m\geq k$ (by hypothesis) and because $m$ takes more weight than $k$ [THIS IS TERRIBLE!!!!!! BUT I'LL FIX IT!!!!!]

All this to say that
\[
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    \leq 
    \frac{2^km^{k/2}k^{k/2}}{(\epsilon m)^k} + o_{x\rightarrow x;\epsilon,m}(1).
\]

Since 
\[
\frac{2^km^{k/2}k^{k/2}}{(\epsilon m)^k}
=
\left(\frac{4k}{\epsilon^2m}\right)^{k/2},
\]
we can optimise this bound by taking $k$ to be the largest even integer less than or equal to $\epsilon^2m/4e$ [just look at the first derivative]. Then:
\[
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    \leq 
    \exp(-\epsilon^2m/C) + o_{x\rightarrow x;\epsilon,m}(1),
\]
with $C=4e\approx 10$. 

\begin{rem}
This bound holds uniformly in $c_1,\dots,c_m$.... VERY IMPORTANT
\end{rem}

Now that we have this bound, note that 
\[
    \PP\left(\sup_{(c_1,\dots,c_m)\in S_m}\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    \leq
    \sum_{(c_1,\dots,c_m)\in S_m}
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right),
\]
which follows by countable additivity of the measure [WHY DO WE EVEN PHRASE IT LIKE THIS?!?!?!?]; in particular
\[
    \PP\left(\sup_{(c_1,\dots,c_m)\in S_m}\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    \leq
    \left(\exp(-\epsilon^2m/C) + o_{x\rightarrow\infty;\epsilon,f}(1)\right)\exp(o_{m\rightarrow\infty;\epsilon,f}(m)),
\]
which follows from the zero entropy hypothesis and from the previous bound.

In particular,
\[
\PP\left(\left|\frac{1}{m}\sum_{i=1}^m f_\epsilon(n+i)\lambda(n+i)\right|\geq \epsilon \right)
\leq
\left(\exp(-\epsilon^2m/C) + o_{x\rightarrow\infty;\epsilon,f}(1)\right)\exp(o_{m\rightarrow\infty;\epsilon,f}(m));
\leq 
\]
taking $m$ sufficiently large (w.r.t. $\epsilon$ and $C$), this can be bounded above by [BE CAREFUL WITH CONSTANTS/DEPENDENCE!!!!!!]
\[
\leq \epsilon + o_{x\rightarrow\infty;m,\epsilon,f}(1).
\]

This then implies that
\[
    \left|\E\left[\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i)\right]\right|
    \leq
    2\varepsilon+\leq o_{x \rightarrow \infty; m,\varepsilon}(1),
\]
which follows by splitting the sum over $n$ according to whether or not the sum over $i$ is $\leq \epsilon$ or $\geq \epsilon$, and then using the previous bound, together with the fact that the summand is bounded in absolute value by $1$.

But, by approximate translation invariance (i.e, over/under-counting),
\[
\E\left[\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i)\right]
=
\frac{1}{x}\sum_{n\leq x}f_\epsilon(n)\lambda(n) + o_{x \rightarrow \infty; m,\varepsilon}(1).
\]

Then, for an appropriate choice of $m$,
\[
\left|\sum_{n\leq x} f_\epsilon(n) \lambda(n)\right|
\leq (o_{x \rightarrow \infty;\epsilon,f}(1) + 2\epsilon) x;
\]
taking this back to estimates for $f$ incurs another error of size $\epsilon x$ so that
\[
\left|\sum_{n\leq x} f(n) \lambda(n)\right|
\leq (o_{x \rightarrow \infty;\epsilon,f}(1) + 3\epsilon) x.
\]
This last bound is equal to $o_{x\rightarrow \infty;f}(x)$ for $\epsilon=\epsilon(x)$ going to $0$ slowly enough w.r.t. $x$.

AND THIS PROVES SARNAK'S CONJECTURE!!!!!!!!!!!!!!!11

We may assume, w.l.o.g., that $f$ is real-valued and bounded by $1$: for complex-valued $f$, we can just split into the real and imaginary parts, respectively, while, for $|f|\leq M$, say, we can simply normalize by $1/M$ to consider $|f|\leq 1$. Let $\epsilon>0$ and, for each $n\in\N$, let $\kappa(n)$ be such that $\epsilon\kappa(n)\leq f(n)<\epsilon(\kappa(n)+1)$. Define $f_\epsilon(n):=\kappa(n)$; i.e., $f_\epsilon$ is $f$ rounded to the nearest multiple of $\epsilon$. Then, 
\begin{align*}
    \left|\sum_{n\leq x}\lambda(n)(f(n)-f_\epsilon(n))\right|
    \leq
    \epsilon x;
\end{align*}
in particular,
\begin{align*}
    \sum_{n\leq x}\lambda(n)f(n)
    =
    \sum_{n\leq x}\lambda(n)f_\epsilon(n) + \mathcal{O}(\epsilon x),
\end{align*}
where we will choose $\epsilon=\epsilon(x)\rightarrow 0$ as $x\rightarrow\infty.$ 

Next, using the that fact $f$ is deterministic, we have that $(f_\epsilon(n+1),f_\epsilon(n+2),\dots,f_\epsilon(n+m))$ takes on at most $\mathcal{O}(\exp(o_{m\rightarrow\infty;f,\epsilon}(m))$ distinct values as $n$ ranges over the positive integers. Let $S_m$ denote the set of these $\exp(o_{m\rightarrow\infty;\epsilon,f}(m))$ possible values. Rather than studying the partial sums of $\lambda f_\epsilon,$ we consider the partial sums of 
\[
\frac{1}{m}\sum_{i=1}^mc_i\lambda(\cdot+i),
\]
where $|c_i|\leq 1$ and where we will eventually take $c_i = f_\epsilon(\cdot + i)$ and then average over $n\leq x$. That is, we are interested in bounding
\[
\frac{1}{x}\sum_{n\leq x}\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i).
\]

In order to evaluate the above, we start by considering 
\begin{align*}
    \#\{n\leq x: \left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon\}.
\end{align*}
From Chebyshev's Inequality, this is bounded above by
\[
\frac{1}{(\epsilon m)^{k}}
\sum_{n\leq x}
\left|\sum_{i=1}^mc_i\lambda(n+i)\right|^{k},
\]
for any $k$ (even), which we are free to choose. By expanding this $k$-th power and using the triangle inequality, we have that
\[
    \#\{n\leq x: \left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon\}
    \leq
    \frac{1}{(\epsilon m)^{k}}\sum_{1\leq i_1,i_2,\dots,i_k\leq m}
    \left|\sum_{n\leq x}\lambda(n+i_1)\lambda(n+i_2)\cdots\lambda(n+i_k)\right|,
\]
which follows by the fact that $|c_i|\leq 1$ for all $i$. By Theorem \ref{main_thm}, the inner sum is
\[
\ll_{k,A} \frac{x}{(\log\log \eta)^A} + o(x)
\]
unless none of the indices $i_1,\dots,i_k$ is repeated an odd number of times and where the implied constant is $\ll (\max_{j}i_j)^{\max_j i^j}\leq m^m$. In the former case, we get a total bound of  
\[
\ll_A \frac{m^mx}{\epsilon^k}\left(\frac{1}{(\log\log \eta)^A} + o(1)\right),
\]
uniformly for $x\in[q^{10},q^{\log\log\eta/3}.$ It remains to count the number of $k$-tuples $(1_i,\dots,i_k)$ for which the indices $i_j$ each have even multiplicity: read the indices from left to right and label $i_j$ as "fresh" if $i_j$ is not equal to any of the indices $i_1,\dots,i_{j-1}$ and label $i_j$ as a "repeat" if otherwise. Given $i_1,\dots,i_{j-1}$, there are at most $m$ choices for $i_j$ if $i_j$ is to be fresh and at most $k$ choices if $i_j$ is a repeat. Furthermore, given $i_1,\dots,i_k$, at most $k/2$ indices are fresh (this is because the multiplicity of each $i_j$ must be even, so that fresh indices actually come with a pair further down the line). Let $N$ denote the number of fresh indices, so that $k-N$ is the number of repeats. Then, there are $2^km^Nk^{k-N}$ possible $k$-tuples with the desired properties and this is $\leq 2^km^{k/2}k^{k/2}$, provided as $m\geq k$. Therefore,
\[
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    \leq 
    \frac{2^km^{k/2}k^{k/2}}{(\epsilon m)^k} + o_{x\rightarrow x;\epsilon,m}(1).
\]
Since 
\[
\frac{2^km^{k/2}k^{k/2}}{(\epsilon m)^k}
=
\left(\frac{4k}{\epsilon^2m}\right)^{k/2},
\]
we can optimise this bound by taking $k$ to be the largest even integer less than or equal to $\epsilon^2m/4e$ [just look at the first derivative], which yields:
\[
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    \leq 
    \exp(-\epsilon^2m/C) + o_{x\rightarrow x;\epsilon,m}(1),
\]
with $C=4e\approx 10$. 

Since the above bound holds uniformly in $c_1,\dots,c_m$, we have that 
\begin{align*}
    \PP\left(\sup_{(c_1,\dots,c_m)\in S_m}\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
    &\leq
    \sum_{(c_1,\dots,c_m)\in S_m}
    \PP\left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)\\
    &\leq
    \left(\exp(-\epsilon^2m/C) + o_{x\rightarrow\infty;\epsilon,f}(1)\right)\exp(o_{m\rightarrow\infty;\epsilon,f}(m)),
\end{align*}
which follows from the zero entropy hypothesis and from the previous bound.

In particular,
\[
\PP\left(\left|\frac{1}{m}\sum_{i=1}^m f_\epsilon(n+i)\lambda(n+i)\right|\geq \epsilon \right)
\leq
\left(\exp(-\epsilon^2m/C) + o_{x\rightarrow\infty;\epsilon,f}(1)\right)\exp(o_{m\rightarrow\infty;\epsilon,f}(m));
\leq 
\]
taking $m$ sufficiently large (w.r.t. $\epsilon$ and $C$), this can be bounded above by [BE CAREFUL WITH CONSTANTS/DEPENDENCE!!!!!!]
\[
\leq \epsilon + o_{x\rightarrow\infty;m,\epsilon,f}(1).
\]

This then implies that
\[
    \left|\E\left[\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i)\right]\right|
    \leq
    2\varepsilon+\leq o_{x \rightarrow \infty; m,\varepsilon}(1),
\]
which follows by splitting the sum over $n$ according to whether or not the sum over $i$ is $\leq \epsilon$ or $\geq \epsilon$, and then using the previous bound, together with the fact that the summand is bounded in absolute value by $1$.

But, by approximate translation invariance (i.e, over/under-counting),
\[
\E\left[\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i)\right]
=
\frac{1}{x}\sum_{n\leq x}f_\epsilon(n)\lambda(n) + o_{x \rightarrow \infty; m,\varepsilon}(1).
\]

Then, for an appropriate choice of $m$,
\[
\left|\sum_{n\leq x} f_\epsilon(n) \lambda(n)\right|
\leq (o_{x \rightarrow \infty;\epsilon,f}(1) + 2\epsilon) x;
\]
taking this back to estimates for $f$ incurs another error of size $\epsilon x$ so that
\[
\left|\sum_{n\leq x} f(n) \lambda(n)\right|
\leq (o_{x \rightarrow \infty;\epsilon,f}(1) + 3\epsilon) x.
\]
This last bound is equal to $o_{x\rightarrow \infty;f}(x)$ for $\epsilon=\epsilon(x)$ going to $0$ slowly enough w.r.t. $x$.

AND THIS PROVES SARNAK'S CONJECTURE!!!!!!!!!!!!!!!11



, by showing that a certain graph which describes divisibility of primes is strong locally expander almost everywhere (as opposed to the work of of Tao and Tao-Ter{\"a}v{\"a}inen, which is based on entropy, not expansion).

%%%%%%
HEATH-BROWN

\begin{proof}
In what follows, we assume that $(\chi_\ell,q_\ell, \beta_\ell)$ is fixed and can thus drop the subscript $\ell$; in particular, let $\chi (\mod q)$ be an exceptional character and suppose $L(\beta_0,\chi)=0$, with $\beta_0=1-1/(\eta\log q)$. The proof follows that of Lemma 3 of \cite{HB_TP}, with one small modification: Heath-Brown stays to the right of the one-line taking $s=1+1/\log q$, which is essentially equal to $s=1+1/\log x$ for $x\in[q^{250},q^{500}]$; since we are dealing with a larger range, we ultimately take $s=1+1/\log x$. We provide the details for the convenience of the reader. 

Let $\Lambda(n)$ denote the von Mangoldt function, which is defined to be $\log p$ if $n$ is a power of a prime $p$ and $0$ otherwise. Then,
\begin{align*}
    \sum_{\substack{{p\leq x}\\{\chi(p)=1}}}\frac{\log p}{p}
    &\leq
    \sum_{\substack{{n\leq x}\\{\chi(n)=1}}}\frac{\Lambda(n)}{n}\\
    &\leq
    \sum_{\substack{{n=1}\\{\chi(n)=1}}}^\infty \frac{\Lambda(n)}{n^s},
\end{align*}
for some $s>1$ to be chosen later. Since $s>1$, this last sum is then bounded above by
\begin{align*}
    \sum_{\substack{{n=1}\\{\chi(n)=1}}}^\infty \frac{\Lambda(n)}{n^s}
    &\leq
    -\frac{\zeta^\prime(s)}{\zeta(s)}-\frac{L^\prime(s,\chi)}{L(s,\chi)}.
\end{align*}

We can now use the explicit formulas to write the RHS in terms of their respective zeros. We begin with the explicit formula for $\zeta$ (see Section 12 of \cite{Davenport}):
\begin{align*}
    \frac{\zeta^\prime(s)}{\zeta(s)}
    &=
    C-\frac{1}{s-1}+\sum_{n=1}^\infty\left(\frac{1}{s+2n}-\frac{1}{2n}\right)+\sum_\rho\left(\frac{1}{s-\rho}+\frac{1}{\rho}\right),
\end{align*}
where the last sum runs over the non-trivial zeros of $\zeta$, where we have combined all constants appearing from equations (8), (9), and (10) in \cite{Davenport} into the constant $C$, and where we have replaced the Gamma factors with a sum over the trivial zeros (which makes bounding things a little easier). In particular, we have that
\begin{align*}
    \frac{\zeta^\prime(2)}{\zeta(2)}-\frac{\zeta^\prime(s)}{\zeta(s)}
    &=
    \frac{1}{s-1}-1 + \sum_{n=1}^\infty\left(\frac{1}{2+2n}-\frac{1}{s+2n}\right)+\sum_{\rho}\left(\frac{1}{2-\rho}-\frac{1}{s-\rho}\right)\\
    &=
    \frac{1}{s-1}+\mathcal{O}(1),
\end{align*}
as both sums converge (with $s\rightarrow 1^+$).

From now on, set $s=1+(\log x)^{-1}$ and $s^\prime=1+a(\log x)^{-1}$, for some $a\gg 1$ to be chosen later. Then, proceeding in the same way as above, we have that
\begin{align*}
    \frac{L^\prime(s^\prime,\chi)}{L(s^\prime,\chi)}
    -
    \frac{L^\prime(s,\chi)}{L(s,\chi)}
    &=
    \sum_{\rho}\left(\frac{1}{s^\prime-\rho}-\frac{1}{s-\rho}\right)
    +
    \mathcal{O}(1),
\end{align*}
where $\rho$ now runs over the non-trivial zeros of the Dirichlet $L$-function associated to $\chi$.

For the term corresponding to $\rho=\beta_0$: note that
\begin{align*}
    |s^\prime-\beta_0|
    &=
    \left|\left(1+\frac{a}{\log x}\right) - \left(1-\frac{1}{\eta\log q}\right)\right|
    =
    \frac{a}{\log x} + \frac{1}{\eta\log q}
    \geq 
    \frac{a}{\log x}
\end{align*}
and that
\begin{align*}
    |s-s^\prime|
    =
    \left|\frac{1}{\log x} - \frac{a}{\log x}\right|
    \ll
    \frac{a}{\log x};
\end{align*}
in particular,
\begin{align*}
    \frac{L^\prime(s^\prime,\chi)}{L(s^\prime,\chi)}
    -
    \frac{L^\prime(s,\chi)}{L(s,\chi)}
    &=
    \frac{1}{s^\prime-\beta_0}
    -
    \frac{1}{s-\beta_0}
    +
    \sum_{\rho\neq \beta_0}\frac{|s-s^\prime|}{|(s^\prime-\rho)(s-\rho)|}
    +
    \mathcal{O}(1)\\
    &\ll
    -
    \frac{1}{s-\beta_0}
    +
    \mathcal{O}\left(
    \frac{\log x}{a}
    +
    \frac{a}{\log x} \sum_{\rho\neq\beta_0}\frac{1}{|\rho-1|^2}
    \right).
\end{align*}

The zeros $\rho=\beta+i\gamma$ for which $\gamma\geq 1$ give a total contribution of
\begin{align*}
    \frac{a}{\log x}\sum_{\substack{{\rho\neq\beta}\\{|\gamma|\geq 1}}}\frac{1}{|\rho-1|^2}
    &\ll
    \frac{a}{\log x}\sum_{\rho}\frac{1}{|\rho-2|^2}
    \ll
    \frac{a\log q}{\log x}
\end{align*}
by Equation (3) of Section 16 in \cite{Davenport}; see also Section 19 of \cite{Davenport}.

For the remaining terms, we can use a result due to Prachar \cite[Lemma 2.1]{Prachar}, which counts the number of zeros of $L(s,\chi)$ in a disk of radius $r\leq 2$, together with a result due to Jutila \cite[Theorem 2]{Jutila}, which Heath-Brown calls the Deuring-Heilbronn phenomenom, which bounds how far away the non-trivial zeros of $L(s,\chi)$ are away from the $1$ line; more precisely, the number of non-trivial zeros of $L(s,\chi)$ in the disk $|s-1|\leq r$ is $\ll 1+r\log q$ when $r\leq 2$, so that the contribution from the zeros $\rho\leq\beta_0$ for which $|\gamma|\leq 1$ is bounded by
\[
\frac{a}{\log x}(1+r_0\log q)r_0^{-2}=\frac{a}{\log x}(r_0^{-2}+r_0^{-1}\log q),
\]
where
\[
r_0:=\min\{|\rho-1|:\rho\neq\beta_0\}\gg \frac{\log \eta}{\log q}.
\]

Therefore,
\[
-\frac{L^\prime(s,\chi)}{L(s,\chi)}
=
\frac{L^\prime(s^\prime,\chi)}{L(s^\prime,\chi)}
-
\frac{1}{s-\beta_0}
+
\mathcal{O}\left(\frac{\log x}{a}+\frac{a\log q}{\log x} + \frac{a(\log q)^2}{(\log x)\log \eta}\right).
\]
But we also have that
\[
\frac{L^\prime(s^\prime,\chi)}{L(s^\prime,\chi)}
\ll
\sum_{n=1}^\infty\frac{\Lambda(n)}{n^{s^\prime}}
\ll
\frac{1}{s^\prime -1}
\ll
\frac{\log x}{a};
\]
in particular, we can now optimize our choice of $a$ (by making the two distinct error terms equal), to get that
\[
\frac{L^\prime(s,\chi)}{L(s,\chi)}
=
-\frac{1}{s-\beta_0}
+
\mathcal{O}((\log q)\log^{-1/2}\eta),
\]
after having made the optimal choice $a=\log^{1/2}\eta$.

Putting all of this together, we have that
\[
\sum_{\substack{{p\leq x}\\{\chi(p)=1}}}\frac{\log p}{p}
=
\frac{1}{s-1}-\frac{1}{s-\beta_0} 
+
\mathcal{O}((\log q)\log^{-1/2}\eta),
\]
with the first term bounded above by
\[
\frac{1}{s-1}-\frac{1}{s-\beta_0} 
=
\frac{2-\beta_0}{(s-1)(s-\beta_0)}
\ll
\frac{(\eta\log q)^{-1}}{(s-1)^2}
\ll
(\log q) \eta^{-1}
\ll
(\log q)\log^{-1/2}\eta
\]
and our claim follows.
\end{proof}

%%%%%%

SARNAK

Before we can get to the proof of Theorem \ref{cor_Sarnak}, we need the following lemma, which is a slight modification to Proposition 5 on Tao's blog (although the proof follows verbatim):
\begin{lem}
\label{High_Probability}
Fix $m\geq 1$ and $\epsilon>0$ and let $c_1,\dots, c_m$ be any numbers on the unit circle. Under the hypotheses of Theorem \ref{main_thm}, 
\[
\frac{1}{x}
\#\left\{n\leq x: \left|\frac{1}{m}\sum_{i=1}^m c_i\lambda(n+i)\right|\geq \epsilon\right\}
\leq
\exp( - \varepsilon^2 m / C ) + o_{x\rightarrow\infty; m,\epsilon}(1),
\]
uniformly for $x\in [q^{10},q^{\log\log\eta/3}]$, where $C$ is an absolute constant and $o_{x\rightarrow\infty;m,\epsilon}(1)$ goes to zero as $x \rightarrow \infty$ (uniformly in the choice of coefficients $c_1,\ldots,c_m$; that is, the implied constant depends only on $\epsilon$ and the number of coefficients, but not on the coefficients themselves).
\end{lem}
\begin{proof}
The proof follows from Chebyshev's Inequality, together with some combinatorics. More precisely, let $k$ be an (even) integer and note that
\begin{align*}
    \#\left\{n\leq x: \left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon\right\}
    &\leq
    \frac{1}{(\epsilon m)^k}\sum_{n\leq x}\left|\sum_{i=1}^m c_i\lambda(n+i)\right|^k\\
    &\leq
    \frac{1}{(\epsilon m)^k}\sum_{1\leq i_1,\dots,i_k\leq m}
    \left|\sum_{n\leq x}\lambda(n+i_1)\cdots \lambda(n+i_k)\right|,
\end{align*}
where the last line follows by expanding the $k$-th power, switching the order of summation, and then passing the absolute value inside, recalling that $|c_i|\leq 1$ for all $i=1,\dots, m$.

The summand can be bounded with the use of Theorem \ref{main_thm}, unless none of $i_j$'s occur with an odd multiplicity, in which case the summand is bounded by $x$ times the number of such tuples $(i_1,\dots,i_k)$. Thus, we simply need to count the number of such tuples and make an appropriate choice for $k$ to conclude the proof of our lemma. Following the proof of Proposition 5 on Tao's blog, we get that the number of such tuples is $\leq 2^km^{k/2}k^{k/2}$, provided $m\geq k$: the idea is to read the indices $i_1,\dots,i_k$ from left to right and to label the index $i_j$ as "fresh" if $i_j\neq i_1,\dots,i_{j-1}$ and "repeat" if otherwise. Since each repeat comes in pairs, there are at most $k/2$ fresh indices and once we fix each index as either fresh or repeat (of which there are $2^k$ such possibilities) and each fixed index will then have at most $m^{k/2}$ fresh choices and $k^{k/2}$ repeats. Thus,
\begin{align*}
    \frac{1}{x}\#\left\{n\leq x: \left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon\right\}
    &\leq
    \left(\frac{4k}{\epsilon^2m}\right)^{k/2} + \frac{1}{\epsilon^k}\left(\frac{m^m C_A}{(\log\log\eta)^A} + o_{x\rightarrow\infty}(m^2) \right),
\end{align*}
uniformly for $x\in[q^{10},q^{\log\log\eta/3}$]. We can optimize the first term by taking $k$ to be the even integer closest to $\epsilon^2m/(4\e)$, which yields that the above is bounded by
\[
    \exp(-\epsilon^2m/C) + o_{x\rightarrow\infty;m,\epsilon}(1),
\]
with $C=8e(\approx 22)$, as claimed.
\end{proof}

With Lemma \ref{High_Probability} in tow, we can now prove Theorem \ref{Sarnak}:
\begin{proof}[Sarnak's Conjecture]
We may assume, w.l.o.g., that $f$ is real-valued and bounded by $1$: for complex-valued $f$, we can split into the real and imaginary parts, respectively; for general bounded $f$, say $|f|\leq M$, we can simply normalize by $1/M$ to consider $|f|\leq 1$. Let $\epsilon>0$ and define $f_\epsilon$ to be equal to $f$ rounded to the nearest multiple of $\epsilon$ while still being bounded in absolutely value by $1$ (it is natural to move from $f$ to $f_\epsilon$ as $f$ is deterministic, so that $f_\epsilon$ already lies in a ball of radius $\epsilon$ and the zero entropy hypothesis is now easier to work with). In particular,
\begin{align*}
    \sum_{n\leq x}\lambda(n)f(n)
    =
    \sum_{n\leq x}\lambda(n)f_\epsilon(n) + \mathcal{O}(\epsilon x)
\end{align*}
and it suffices to show that $\lambda$ is orthogonal to $f_\epsilon$, for some $\epsilon=\epsilon(x)\rightarrow 0$ as $x\rightarrow\infty$. 

The idea now is to introduce some shifts in our summand in order to apply Chowla's Conjecture. By the approximate "translation invariance" of our partial sums, and from the fact that everything is one-bounded by hypothesis, we have that
\[
\sum_{n\leq x}f_\epsilon(n)\lambda(n)
=
\sum_{n\leq x}\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i) + \mathcal{O}(m),
\]
for any $m\geq 1$. Furthermore, we can split the sum over $n$ on the RHS according to whether or not the summand is $\leq \epsilon$ or $\geq \epsilon,$ respectively, to get that
\begin{align}
\label{shifted sum}
    \sum_{n\leq x}\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i)
    =
    \sideset{}{'}\sum_{n\leq x}\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i) + \mathcal{O}(\epsilon x),
\end{align}
where the $'$ indicates that we are summing over the integers $n\leq x$ such that 
\[
\left|\frac{1}{m}\sum_{i=1}^mf_\epsilon(n+i)\lambda(n+i)\right|\geq \epsilon
\]
and it now suffices to count how many such $n$ exist. To this end, recall that $f$ is deterministic; in particular, $(f_\epsilon(n+1),f_\epsilon(n+2),\dots,f_\epsilon(n+m))$ takes on at most $\mathcal{O}(\exp(o_{m\rightarrow\infty;f,\epsilon}(m))$ distinct values as $n$ ranges over the positive integers. So, let $S_m$ denote the set of these $\exp(o_{m\rightarrow\infty;\epsilon,f}(m))$ possible values and note that
\begin{align*}
    \#\left\{n\leq x:
    \sup_{(c_1,\dots,c_m)\in S_m}\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon
    \right\}
    &\leq
    \sum_{(c_1,\dots,c_m)\in S_m}
     \#\left\{n\leq x:
     \left(\left|\frac{1}{m}\sum_{i=1}^mc_i\lambda(n+i)\right|\geq \epsilon \right)
     \right\}\\
     &\leq x\left(\exp(-\epsilon^2m/C) + o_{x\rightarrow\infty;m,\epsilon}(1)\right)\exp(o_{m\rightarrow\infty;\epsilon,f}(m)),
\end{align*}
where the last line follows from Lemma \ref{High_Probability} together with the zero entropy hypothesis. In particular,
\begin{align*}
\#\left\{
n\leq x:
\left|\frac{1}{m}\sum_{i=1}^m f_\epsilon(n+i)\lambda(n+i)\right|\geq \epsilon \right\}
&\leq
x\left(\exp(-\epsilon^2m/C) + o_{x\rightarrow\infty;\epsilon,f}(1)\right)\exp(o_{m\rightarrow\infty;\epsilon,f}(m))\\
&\leq 
x(\epsilon + o_{x\rightarrow \infty;\epsilon,f}(1))
\end{align*}
which follows by taking $m$ sufficiently large w.r.t. $\epsilon$ and $C$. Upon inserting the last bound into Equation \ref{shifted sum}, we obtain the desired resulted, provided $\epsilon=\epsilon(x)\rightarrow \infty$ slowly enough with respect to both $x$ and $\eta$.
\end{proof}



%%%%%%

In this section. we prove Corollary \ref{cor_Sarnak}; namely, 
\[
\text{Siegel zeros} \Rightarrow \text{Chowla's Conjecture} \Rightarrow \text{Sarnak's Conjecture}.
\]
More precisely,
\begin{thm}
\label{Sarnak}
Assuming the existence of Siegel zeros, Sarnak's Conjecture holds along a subsequence.
\end{thm}

A conjecture due to Sarnak states that the Liouville function is orthogonal to every deterministic sequence, which can be viewed as a special case of the so-called "M{\"o}bius Randomness Law" \cite[Section 13]{IwaKow}. More precisely, Sarnak's Conjecture states the following:

we are more interested in understanding the relationship between Siegel zeros and Sarnak's Conjecture. To this end, recall the following definition:
Using a well-known argument due to Sarnak, we can now deduce Sarnak's Conjecture on M{\"o}bius disjointness:

%%%%%%%%%%%%%%%%%%%%%%%%%

The sum over the higher prime powers can be bounded trivially:
\begin{align*}
    x\sum_{\substack{{p^\alpha\leq x}\\{p> r}\\{\alpha\geq 2}}}\frac{|\lambda(p^\alpha)-\chi(p^\alpha)|}{p^\alpha}
    &\ll
    x\sum_{p>r}\sum_{\alpha\geq 2}\frac{1}{p^\alpha}\\
    &\ll
    x\sum_{p>r}\frac{1}{p^2}\frac{1}{1-\frac{1}{p}}\\
    &\asymp
    x\sum_{p>r}\frac{1}{p^2}\\
    &\ll
    \frac{x}{r}.
\end{align*}

%%%%%%%%%%%%%%%%
\begin{align*}
    \frac{x}{\log r}&\left(\exp\left(\frac{\log x}{\log q}\right)(\log q)\log^{-1/2}\eta
    +
    \log\log q\right)
    +
    \frac{x}{r}\\
    &=
    \frac{x\log\log\eta}{\log x}\left(
    \exp\left(\frac{\log\log\eta}{3}\right)(\log x)\log^{-1/2}\eta
    +
    \log\log x
    \right)
    +
    x^{1-1/\log\log\eta}\\
    &=
    \frac{x\log\log\eta}{\log^{1/6}\eta} 
    +
    \frac{x\log\log\eta\log\log x}{\log x} 
    +
    x^{1-1/\log\log\eta}.
\end{align*}

Finally, using the bound $\eta\ll q$ (Siegel's Theorem: Equation \ref{Siegel}), we have that
\begin{align*}
    \frac{x\log\log\eta\log\log x}{\log x} 
    \leq
    \frac{x(\log\log x)^2}{\log x},
\end{align*}
which produces an admissible error, while
\begin{align*}
    x^{1-1/\log\log\eta}
    &=
    x\exp\left(\frac{-\log x}{\log\log\eta}\right)\\
    &\ll
    x\exp\left(\frac{-10\log q}{\log\log \eta}\right)\\
    &\ll
    x\exp\left(\frac{-10\log \eta}{\log\log \eta}\right)\\
    &\ll
    \frac{x}{\log \eta},
\end{align*}
where the last bound is arbitrary and again produces an admissible error.

Hence,
\begin{align*}
    \frac{1}{x}\sum_{n\leq x}\lambda(n;k)
    =
    \frac{1}{x}\sum_{n\leq x}\lambda_r(n;k)
    +
    \mathcal{O}_k\left(\frac{\log\log \eta}{(\log\eta)^{1/6}}\right),
\end{align*}
as claimed.
